Open Evaluation Tool for Layout Analysis of Document Images

This paper presents an open tool for standardizing the evaluation process of the layout analysis task of document images at pixel level. We introduce a new evaluation tool that is both available as a standalone Java application and as a RESTful web service. This evaluation tool is free and open-source in order to be a common tool that anyone can use and contribute to. It aims at providing as many metrics as possible to investigate layout analysis predictions, and also provide an easy way of visualizing the results. This tool evaluates document segmentation at pixel level, and support multi-labeled pixel ground truth. Finally, this tool has been successfully used for the ICDAR2017 competition on Layout Analysis for Challenging Medieval Manuscripts.

==> OSTreviews.tex <==

----------------------- REVIEW 1 ---------------------
PAPER: 9
TITLE: Open Evaluation Tool for Layout Analysis of Document Images
AUTHORS: Michele Alberti, Manuel Bouillon and Rolf Ingold

Overall evaluation: 2 (accept)

----------- Overall evaluation -----------
This paper presents an open-source evaluation tool for pixel-level annotation of document images.
The topic is interesting, and fits perfectly the scope of OST.

The paper needs a further proofreading step, since several spelling errors are still present, e.g.:
- at pixel level, and support(S)
- Its goad (GOAL) is to 
- which mean(S) that
- anyone can used (USE) it
etc.

The discussion of the different metrics in Section III is well presented, though maybe some details are obvious for many potential readers (but I understand its presence for the sake of completeness).
I missed however a little review of the state of the art. Are there other freely available tools? (I'm quite sure there are from past competitions). Which are their drawbacks? Why should anyone choose to use yours? etc. It would be nice to motivate your work in this sense apart the fact that having such open source tools available is cool.

Finally, from reading the paper it was not clear to me if the tool is expecting a particular kind of input (labels) that is predefined by your competition or if it can accept any kind an number of different labels as GT input and expected output. If this is the case, I think that you should point that clearly, since it is a strong selling point, that your tool has been tested in the context of historical documents but could be used in any other pixel-level classification scenario, e.g. administrative documents, text detection in real scenes, etc.

----------- Originality (for original software papers only) -----------
Very few details on how to use the tool are present in the paper, although I have the impression that with the selected architecture (java code and restful WS) it should be straightforward for anyone to plug and play.


----------------------- REVIEW 2 ---------------------
PAPER: 9
TITLE: Open Evaluation Tool for Layout Analysis of Document Images
AUTHORS: Michele Alberti, Manuel Bouillon and Rolf Ingold

Overall evaluation: 3 (strong accept)

----------- Overall evaluation -----------
Proposal fits all the objective of the workshop ( OpenSource, web service access ) and this tools was used for the segmentation competition. It includes several metrics form various experiences in the past. This is useful to produce measures that can be compared with other publications.

It really makes sense to be demonstrated and discussed during the workshop.


----------------------- REVIEW 3 ---------------------
PAPER: 9
TITLE: Open Evaluation Tool for Layout Analysis of Document Images
AUTHORS: Michele Alberti, Manuel Bouillon and Rolf Ingold

Overall evaluation: 2 (accept)

----------- Overall evaluation -----------
This paper complies with the openness requirements, fits in the topics of ICDAR, and is potentially useful.


----------------------- REVIEW 4 ---------------------
PAPER: 9
TITLE: Open Evaluation Tool for Layout Analysis of Document Images
AUTHORS: Michele Alberti, Manuel Bouillon and Rolf Ingold

Overall evaluation: 1 (weak accept)

----------- Overall evaluation -----------
We agree with the authors that evaluation tools should by all means be publicly available and Open Source. Therefore it is a pity that the tool has no real brand name (it is obviously part of the DIVA services) since authors claim that it runs as a standalone tool as well. The choice for pixel level evaluation can be justified with the argument that it allows for the most accurate evaluation methods. On the other hand the generation of Ground Truth might be in many cases rather laborious and therefore expensive. 
We also support the idea that several metrics shall be offered since the “best” method might not always be the optimal method for a given problem. In this context it would maybe be helpful to get a bit more details why authors are preferring the Jaccard Index, maybe connected with some real world figures.
There are several typos and grammatical errors (e.g. missing third person s) in the text which needs to be carefully proof-read. Also sometimes the paper uses a bit too much “marketing” slang, e.g. the word “very” is used definitely too often: „very easy“ (2x), „very common task“, „very interesting“, „very impractical“, „very straightforward“, „very human-friendly“.

Finally reviewer got the hint from a colleague that there is an error in the definition of L, cf., p2. Here the statement in detail: The definition of L as a set contradicts its usage. A set has no order and no repeated elements, which are frequently present in your case (different pixels can be labeled equally). 
Since a set has no order you can not refer to an element of L by L_i. 
We suggest to introduce L as a n-tupel whose entries are subsets of C (elements of the power set of C). 
Therefore, L is element of (2^C)^n  (it is element of the cartesian product of n-times the power set of C): 
L\in\mathscr{P}(C)^n

